Learning-Based Adaptive IRS Control with Limited Feedback Codebooks

Intelligent reflecting surfaces (IRS) consist of configurable meta-atoms, which can change the wireless propagation environment through design of their reflection coefficients. We consider a practical setting where (i) the IRS reflection coefficients are achieved by adjusting tunable elements embedded in the meta-atoms, (ii) the IRS reflection coefficients are affected by the incident angles of the incoming signals, (iii) the IRS is deployed in multi-path, time-varying channels, and (iv) the feedback link from the base station to the IRS has a low data rate. Conventional optimization-based IRS control protocols, which rely on channel estimation and conveying the optimized variables to the IRS, are not applicable in this setting due to the difficulty of channel estimation and the low feedback rate. Therefore, we develop a novel adaptive codebook-based limited feedback protocol where only a codeword index is transferred to the IRS. We propose two solutions for adaptive codebook design: random adjacency (RA) and deep neural network policy-based IRS control (DPIC), both of which only require the end-to-end compound channels. We further develop several augmented schemes based on the RA and DPIC. Numerical evaluations show that the data rate and average data rate over one coherence time are improved substantially by our schemes.

==> IRS.tex <==
% \vspace{-1.5mm}
\subsection{Practical Considerations for Intelligent Reflecting Surface}
\label{ssec:IRS}


An intelligent reflecting surface (IRS) represents a {\it software-controlled meta-surface}.\footnote{Since its name is not standardized, it is called many other different names, such as reconfigurable intelligent surface (RIS), intelligent reflective surfaces, or programmable meta-surface.} An IRS is composed of two interconnected systems: a meta-surface  as a physical core and a control circuit as an algorithm core. 
%We  discuss each of them in Sec. III-A and B, respectively. Then, we discuss  two practical considerations for the reflection behaviors of IRS elements in Sec. III-C.
%
%
%In this paper, we refer IRS as an entire structure that has both the meta-surface and control circuit.
%
%
%In this section, we first focus on the physical core, describe the physics/behavior of meta-surface in Sec. \ref{subsec:physics}, and the properties of practical reflection coefficients in Sec. \ref{subsec:prac}. 
%Then, we focus on the algorithm core, discuss a real-time IRS control in Sec. \ref{subsec:IRScontrol}, and an adaptive codebook strategy in Sec. \ref{subsec:codebook}. 
%
%
%\subsection{Meta-surface as a Physical Core}
%\label{subsec:physics}
%\textbf{Meta-surface and meta-atoms.} 
First, as a physical core, a meta-surface is a metallic surface that is composed of meta-atoms (unit element), where each meta-atom size is in subwavelength, typically from $\lambda/10$ to $\lambda/2$, where $\lambda$ denotes the wavelength of the signal. 
Each {\it meta}-atom can change its behavior, such that it absorbs, reflects, refracts, and changes the polarization of the incoming signals. 
The meta-atoms contain tunable elements, such as positive-intrinsic-negative (PIN) diodes, variable capacitors (varactors), memristors, and microelectromechanical systems (MEMS). 
Recent researches, e.g., \cite{abeywickrama2020intelligent,zhu2013active, tang2020wireless,cai2020practical,chen2020angle}, focus on the varactor-implemented meta-atom, since the varactor can offer each meta-atom almost a full $360^o$ reflection phase \cite{zhu2013active}.
In this paper, we consider the varactors as tuning elements.
%
%\textbf{Physics of meta-surface.} 
%On {\it{any}} metallic surface, incoming signals  induce electric current, i.e., motion of electrons, on the metallic surface. Then, the induced current radiates the electromagnetic wave, which is the reflected signal from the surface.
%In case of the {\it meta}-surface, the reflecting behavior can be changed in a desired way.
By tuning the capacitances of varactors, we can adjust the impedances over the meta-surface, and therefore change the electric current on the surface. With a proper tuning of elements, the signals would become constructive at a desired angle, and thus a beamforming is achieved. 

%\subsection{Control Circuit as an Algorithm Core}
%\label{subsec:physics}

For the control circuits, current developments generally account for a field programmable gate array (FPGA)~\cite{yang2016programmable,zhang2018space,abadal2020programmable} as an algorithm core.
In this paper, we adopt the FPGA-based control circuit.
%
%, which is connected to the meta-surface (physical core) to control the varactors
Specifically, the meta-surface (physical core) is connected to the FPGA (algorithm core) via connectors so that the varactors are controlled by the FPGA-based circuit signals (See Fig.6 (a) in \cite{abadal2020programmable}).
%
%We have so far investigated the reflection coefficient on a single unit element of meta-surface, i.e., $\phi(C, \theta)$. 
%For $N_{\rm IRS}$ units,
%the reflection coefficient of $n$-th unit is represented as $\phi(C_n, \theta)$. 
%Including the time index $t$, we can represent the reflection coefficient as $\phi(C_n[t], \theta[t])$, considering that the channels are varying and capacitance is a variable parameter.
%
%The IRS reflection matrix
%${\boldsymbol \Phi}( {\bf c}[t] , \theta[t] ) = {\rm diag} (\phi(C_1[t], \theta[t]),  ..., \phi(C_{N_{\rm IRS}}[t], \theta[t]))$,
%which represents the reflection coefficients of all $N_{\rm IRS}$ elements, is controlled by the capacitances vector ${\bf c}[t] = [ C_1[t], ..., C_{N_{\rm IRS}}[t] ]$, which is the collection of all capacitances on IRS.
%
%The reflection coefficient of $n$-th element is controlled by the variable capacitance $C_n[t]$.
%Specifically, 
The capacitance $C_n[t]$ is controlled by a bias voltage applied to the corresponding unit element.
%, normally with the relationship \cite{} as
%$C_n[t] \propto 1/\sqrt{V_n[t]}$.
Given that the applied voltage ranges between $0$ and $V_{\max}$, the capacitance ranges between $C_{\min}$ and $C_{\max}$, implying:
\begin{equation}
    C_{\min} \le C_{n}[t] \le C_{\max},
    \label{eq:Crange}
\end{equation}
where $C_{\min}$ and $C_{\max}$ varies for the types of varactors embedded in the meta-surface.

\rev{Add a reason why we control capacitances and explain it is a common approach, etc.}

\rev{Add a figure to explain the reflection coefficient controlled by capacitance}



%\subsection{Reflection Coefficient as a Function of Incident Angle and Capacitance}
%\label{subsec:prac}

The reflection coefficient varies from the variable capacitances. Also, the reflection coefficient is found to be varying from the incident angles of the incoming signals  \cite{tang2020wireless,chen2020angle,pei2021ris,zhang2020controlling,costa2020metamaterials,costa2021electromagnetic}. 
%Let us take a look at its mathematical representation using the equivalent circuit model as below.
%
%
%
As the physical size of the unit element is usually smaller than the wavelength of the incident signal, the signal response can be described by an equivalent circuit model of the unit element \cite{koziel2013surrogate}, shown in other works, e.g., \cite{chen2020angle,pei2021ris,costa2021electromagnetic}.
With an equivalent circuit model, the reflection coefficient of each unit element can be expressed as
%It can be also expressed using the equivalent circuit model.
%When using the equivalent circuit model, 
%Then, the reflection coefficient 
%can be expressed as
\begin{equation}
    \phi(C_n[t], \theta[t]) = \frac{Z(C_n[t], \theta[t]) - Z_0}
    {Z(C_n[t], \theta[t]) + Z_0},
    \label{eq:reflectioncoeff}
\end{equation}
where $Z(C_n[t], \theta[t])$ is the impedance of the $n$-th element and $Z_0 \approx $ \SI{376.73}{\ohm} is the impedance of free space.
%
Here, $Z(C_n[t], \theta[t])$ is determined by the incident angle and variable capacitance.
%
We adopt the symmetrical metallic patches brided by a varactor diode according to the work \cite{chen2020angle}. 
In such unit element structure, the equivalent virtual elements $R_1(\theta[t]), L_1(\theta[t]), C_1(\theta[t]), L_2(\theta[t])$ are introduced for equivalent circuit model. Depending on the physical structure of unit element, the composition of virtual elements is determined.
The values of the virtual elements are determined by the {\it projected} geometry on the meta-surface \cite{chen2020angle}.
%
Then, the impedance\footnote{In fact, the impedance $Z$ is also dependent on the angular frequency $\omega$ in \eqref{eq:Z}, i.e., $Z(C_n[t], \theta[t], \omega)$. 
We can approximate
the phase response as constant if the signal bandwidth $W$ is limited to a few tens of MHz, as shown in the plots of the reflection coefficients along $w$ in the works, e.g.,  \cite{chen2020angle,pei2021ris}.
In this paper, we consider a fixed operating frequency and narrowband with a few tens of MHz, and therefore we do not consider the dependency of $\omega$.
%
Also, strictly speaking, the incident angle $\theta[t]$ is  dependent on the operating frequency, because the channel propagation varies in frequencies of the propagating signals. In this paper, since we consider a narrowband signal, it is reasonable to assume that the channel properties including the angles are the same across the utilized frequency band.} $Z(C_n[t], \theta[t])$ of such equivalent circuit is expressed as follows:
\begin{equation}
    Z(C_n[t], \theta[t]) =
    \frac{j\omega L_2(\theta[t]) \big( R_1(\theta[t]) + j\omega L_1(\theta[t]) + \frac{1}{j \omega C_1(\theta[t])}   + \frac{1}{j \omega C_n[t]} \big) }
    {
    j\omega L_2(\theta[t]) + \big( R_1(\theta[t]) + j\omega L_1(\theta[t]) + \frac{1}{j \omega C_1(\theta[t])}   + \frac{1}{j \omega C_n[t]} \big)    
    },
    \label{eq:Z}
\end{equation}
where $\omega = 2 \pi f_c$ is the angular frequency of the incident waves.
%
%
%
%In \cite{zhu2013active}, the incident waves are assumed to be impinging normally on the meta-surface, and therefore the virtual elements are not function of incident angle $\theta$. However, 
%In \cite{chen2020angle}, it was shown that the virtual elements are the function of incident angle $\theta$ due to the fact that the parameter values of the equivalent virtual elements are determined by {\it projected} geometry on meta-surface.
%As a result, the impedance $Z(C, \theta)$ is a function of the incident angle as well as the variable capacitance. 
%
%Then, the reflection coefficient 
%can be expressed as
%\begin{equation}
%    \phi(C, \theta) = \frac{Z(C, \theta) - Z_0}
%    {Z(C, \theta) + Z_0},
%    \label{eq:reflectioncoeff}
%\end{equation}
%where $Z(C, \theta)$ is given in \eqref{eq:Z} and $Z_0 \approx $ \SI{376.73}{\ohm} is the impedance of free space.
%
From \eqref{eq:reflectioncoeff} and \eqref{eq:Z},
we can figure out two important considerations for the practical reflection behaviors of the IRS equipped with varactors.
% expression in \eqref{eq:reflectioncoeff}.


\begin{itemize}
\item {\it Consideration 1. Dependency between amplitude and phase shift.}
The amplitude $|\phi(C_n[t], \theta[t])|$ and phase shift $\angle \phi(C_n[t], \theta[t])$ is jointly controlled by the variable capacitance $C_n[t]$. In other words, the amplitude and the phase shift cannot be controlled independently in practice.
%The amplitude $|\phi(C_n[t], \theta)|$ and the phase shift $\angle \phi(C_n[t], \theta)$ of meta-atom cannot be independently controlled, while those of conventional antenna elements are controlled independently due to the separate hardware of the attenuator and phase shifter.

%In recent work \cite{abeywickrama2020intelligent}, the authors proposed a practical phase shift model, where the dependency between the amplitude and the phase shift is considered for a beamforming design.

\item {\it Consideration 2. Reflection coefficient dependent on incident angle.}
The reflection coefficient $\phi(C_n[t], \theta[t])$ is also a function of the incident angle $\theta[t]$. 
%signals from different path will have different response on the same IRS unit cell.
In other words, incoming signals from different paths will experience different responses on the same IRS unit element.
Under the practical channel conditions of (i) multiple signals with different angles and (ii) time-varying nature of angles, it would be challenging to optimize the capacitances in real-time.
Furthermore, in uplink, UE-IRS channels are more susceptible to vary because of the mobility of UE and scatterers.
\end{itemize}


From Consideration 1, it is natural to control the variable capacitances, instead of the reflection coefficients directly, because some reflection coefficient values may not be achievable.
From Consideration 2, in order to optimize for the capacitances, the BS is required to be informed of a huge amount of information/estimates (e.g., the function of $Z(\cdot)$ for every capacitance and angle, the incident angles and path gains for each signal path of the UE-IRS channel) with IRS-BS channel and UE-BS channel for {\it every} coherence time. Practically, the incident angles and path gains for each signal path of the UE-IRS channel are unmeasurable because the IRS is a passive equipment.
Furthermore, the channels of UE-IRS and IRS-BS  cannot be measured with unexpected incident angles.

%In this paper, we consider that the BS employ a channel-free method without any channel information, or a learning method with limited channel information, i.e., a few of effective channels,
%instead of estimating all the aforementioned information.

%reflection coefficients cannot be predicted nor formulated in practical channel conditions, i.e., dynamic channels with NLOS incoming signals.
%%Therefore, in this paper, we will design the configuration of capacitances over meta-surface, instead of reflection coefficients.
%Further, we consider that we only measure the effective channels as available information for designing variables, instead of measuring all the individual channels and incoming signals.


%So far, we have investigated the reflection coefficient, in practice, as a function of 
%The objective of this paper is to control the collection of variable capacitances $C$ over meta-surface under aforementioned two practical considerations.
%However, due to the challenges of acquiring the individual channels (UE-BS, UE-IRS, and IRS-BS) and estimating the incident angles in real-time under a dynamic environment, we cannot use any mathematical formulation




%




%We consider an IRS update over time by controlling IRS capacitances ${\bf c}[t]$. 


%The reconfigurability of IRS is accomplished by controller. 
%In this paper, we adopt the FPGA-based control circuit as IRS controller to align with recent developments of practical implementation and its several advantages. 
%The FPGA-based control circuit enables the algorithm core to be designed independently from meta-surface, which is beneficial to the function expansion and performance upgrade of the entire system by just changing the FPGA programs without modifying the physical structure of meta-surface.



%\textbf{Coding meta-surface.}  With FPGA, the concept of  coding meta-surfaces was initially proposed in \cite{cui2014coding}, and has rapidly evolved \cite{zhang2018space,yang2016programmable,sun2020infrared}. The designed coding sequences are first stored in FPGA, and then the desired coding sequence can be selected adaptively  for a desired beamforming in real time. 
%%The coding schemes for meta-surface control are used in several forms of tuning elements, such as PIN diodes \cite{zhang2018space,yang2016programmable} and varactor \cite{sun2020infrared}.
%%For example, in case of varactors for tuning elements \cite{sun2020infrared}, 
%%a 1-bit coding metasurface is constructed by a sequence of 0 or 1, exhibiting 0 or 180 (deg) by mapping the bit (0 or 1) to a proper capacitance that leads to a desired phase shift (0 or 180 deg).
%%In \cite{sun2020infrared} capacitances are set as 2.67 and 0.73 pF, so to have 0 or 180 (deg) phase responses.
%For tuning the varactors \cite{sun2020infrared}, a 1-bit coding metasurface is constructed by a sequence of 0 or 1, each exhibiting 0 or 180 (deg). This is achieved by mapping the bit (0 or 1) to  proper capacitances (2.67 and 0.73 pF in \cite{sun2020infrared}) leading to 0 or 180 (deg).
%This coding meta-surface provides a powerful tool in functional metasurface design by building a bridge between the physical and digital worlds.
%However, for $N_{\rm IRS}$ elements, we have total $2^{N_{\rm IRS}}$ distinct coding sequences to consider, which still causes computational burden to decide a proper coding sequence with large numbers of meta-surface elements \cite{yang2016programmable}. Also, it may be inefficient to only consider 0 or 180 (deg) as reflection phase.
%%One way to mitigate the computational burden is to group the metasurface region into several sub-array, and control the sub-array with common signals at the expense of beam accuracy \cite{sun2020infrared}.



%\textbf{Switching speed of reconfiguration.} 
%Coding meta-surface enables a real-time control for IRS reconfiguration by storing a finite set of coding sequences in FPGA.
%The switching speed of reconfiguration is typically known for a few kHz (hundreds of $\mu s$) \cite{abadal2020programmable, sun2020infrared}. Specifically, the switching speed will be determined by the characteristics of the FPGA-based control circuits and by how it communicates with the metasurface.
%Considering the channel coherence time is a few $ms$ following a cellular standard \cite{ieeep80216}, the meta-surface can be sufficiently reconfigured in real-time because the switching speed is faster than the coherence time. 




%\subsection{Proposed IRS Control Scheme in Short-term and Long-term
%% Adaptive Codebook Update via  Reprogramming FPGA
%}
%\label{subsec:codebook}


%In this paper, we adopt a codebook strategy, where the codebook is implemented/stored in the FPGA. The codebook is a finite set of  realizable capacitances on meta-surface, $\mathcal{C} = \{ {\bf c}_i\}_{i=1}^{N_c} $ with size $|\mathcal{C}| = N_{c}$.
%%This is different from choosing a coding sequence from $2^{N_{\rm IRS}}$ distinct coding sequences. 
%Each codeword vector in the codebook represents the collection of capacitances over meta-surface, i.e., ${\bf c}_i = [ C_{i,1}, ..., C_{i,N_{\rm IRS}} ], \forall i$, which forms a specific reflection coefficient matrix.
%Compared to conventional digital coding meta-surface strategy focusing on bits coding of each meta-atom, we focus on designing the collection of capacitances over meta-surface as a codeword.
%The codebook design strategy will reduce the computational complexity just by choosing index of corresponding codeword in codebook. 
%%Typically, the codebook size will be smaller than the number of distinct coding sequences
%% in the case of large numbers of meta-surface elements, 
%%by having the codebook size as, $N_{c} \ll 2^{N_{\rm IRS}}$.

%\textbf{IRS capacitances update in short-term (real-time).}
%Because IRS often does not have sensing capabilities, it cannot actively select the capacitance vector ${\bf c}[t]$ according to the environment dynamics. 
%%A common approach for IRS control is to use an external communication link from BS to IRS, where BS transmits an information for control. 
%In this paper, we assume a limited feedback link for the BS to send the index $i[t]$ of the corresponding codeword in the codebook, where the codebook is shared both at BS and IRS.


%\textbf{Codebook update in long-term.}
%The FPGA-based control circuit enables the algorithm core to be designed independently from meta-surface, which is beneficial to the function expansion and performance upgrade of the entire system by just changing the FPGA programs without modifying the physical structure of meta-surface.
%The initially constructed codebook may be outdated by varying environments over time, leading to performance degradation because the codebook may no longer provide a good solution space for meta-surface capacitances.
%%
%Therefore, we propose an adaptive codebook design strategy via reprogramming FPGA. 
%%Evolving codebook will perform better than static codebook.
%The FPGA reprogram for codebook update can be done via communication link with BS. However, the reprogramming of FPGA should not be too often due to the reprogramming cost with respect to the reprogramming time and communication overhead for update. 
%Therefore, we consider that the codebook update is a long-term update, while the IRS capacitances update is a short-term (real-time) update.


%\clearpage
